Exploiting Row-Level Temporal Locality in DRAM to Reduce the Memory Access Latency

This paper summarizes the idea of ChargeCache, which was published in HPCA 2016 [51], and examines the work's significance and future potential. DRAM latency continues to be a critical bottleneck for system performance. In this work, we develop a low-cost mechanism, called ChargeCache, that enables faster access to recently-accessed rows in DRAM, with no modifications to DRAM chips. Our mechanism is based on the key observation that a recently-accessed row has more charge and thus the following access to the same row can be performed faster. To exploit this observation, we propose to track the addresses of recently-accessed rows in a table in the memory controller. If a later DRAM request hits in that table, the memory controller uses lower timing parameters, leading to reduced DRAM latency. Row addresses are removed from the table after a specified duration to ensure rows that have leaked too much charge are not accessed with lower latency. We evaluate ChargeCache on a wide variety of workloads and show that it provides significant performance and energy benefits for both single-core and multi-core systems.

==> sections/test_of_time.tex <==
\section{Test of Time Award Citation}

Utilizing the main memory access behavior of the applications to
reduce DRAM latency has inspired a wide range of ideas in the
field of memory systems.  Over the past decade, the key
observations made in this paper have pioneered the research in
memory performance and reliability. 



